Nuclear medium effects in Drell-Yan process

We study the nuclear medium effects in Drell-Yan process using quark parton distribution functions calculated in a microscopic nuclear model which takes into account the effects of Fermi motion, nuclear binding and nucleon correlations through a relativistic nucleon spectral function. The contributions of $\pi$ and $\rho$ mesons as well as shadowing effects are also included. The beam energy loss is calculated using a phenomenological approach. The present theoretical results are compared with the experimental results of E772 and E886 experiments. These results are applicable to the forthcoming experimental analysis of E906 Sea Quest experiment at Fermi Lab.

==> sortbib <==
#!/usr/bin/perl -w
# 1) Save this script into a file called sortbib.
# 2) Type chmod 755 sortbib.
# 3) Change the first line to identify the location of perl on your
#    machine. (Type "which perl" or "whereis perl".) 
# 4) Take a Latex file which uses \cite{} to reference \bibitem{}'s,
#    and type sortbib file.tex.

# Written by Steven R. White
# Usage: sortbib latexfile.tex
# Sort \bibitems in order by \cites
# Comments out unused bibitems, reports on citations without references,
# and makes a backup file file.tex.bak.
# sortbib understands Latex comments, and doesn't get fooled
# by \%, etc.

$\ = "\n";		# set output record separator

sub removecomments	# comments: %, \\%, \\\\%, etc
    {			# not comments: \%, \\\%, etc
    $_[0] =~ s/\\\\/\xbb\xbb/g;	# Change double \ to weird chars
    $_[0] =~ s/\\\%/\xcc\xcc/g;	# Change \% to weird chars
    $_[0] =~ s/\%[^\n]*\n//g;
    $_[0] =~ s/\xcc\xcc/\\\%/g; # Change back
    $_[0] =~ s/\xbb\xbb/\\\\/g;
    }

sub getcomments
    {
    local($txt) = @_;
    $txt =~ s/\\\\/\xbb\xbb/g;
    $txt =~ s/\\\%/\xcc\xcc/g;
    @bibco = ($txt =~ /(\%[^\n]*\n)/g);
    for($i=0; $i <= $#bibco; $i++)
	{
	$bibco[$i] =~ s/\xcc\xcc/\\\%/g;
	$bibco[$i] =~ s/\xbb\xbb/\\\\/g;
	}
    @bibco;
    }

foreach $file (@ARGV) 
    {
    `cp $file $file.bak`;
    open(FILE,"<$file");
    undef $/;
    $wholefile = <FILE>;
    close FILE;
    open(OUT,">sortbib.tmp");
    $dothebib = ($wholefile =~ /thebibliography/);
    $bibpat = '';
    if($dothebib)
	{
	$wholefile =~ /(\\begin\{thebibliography\}\{\d+\})/;
	$bibpat = $1;
	@fileparts = split( 
	/\\begin\{thebibliography\}\{\d+\}|\\end\{thebibliography\}/,
    				$wholefile,3);
	}
    else
	{
	$bibpat = "\\begin\{references\}";
	@fileparts = split( /\\begin\{references\}|\\end\{references\}/,
    				$wholefile,3);
	}
    $text = $fileparts[0];
    $text =~ s/\n+$/\n/;
    print OUT $text;
    &removecomments($text);
    $text =~ s/onlinecite/cite/g;

    @cites = ($text =~ /\\cite\{([^\}]*)\}/g);
    @citelist = split(/[\s\,]+/,join(",",@cites));
    @uniquecites = ();
    foreach $ci (@citelist)
	{
	push(@uniquecites,$ci) if !grep(/^$ci$/,@uniquecites);
	}
    $list = join("\n",@uniquecites);
    print "Citations:";
    print $list;
    print "";

    $references = $fileparts[1];
    @bibco = &getcomments($references);
    &removecomments($references);
    $references =~ s/\n\n/\n/g;
    @bibitems = split(/\\bibitem/,$references);
    %bibhash = ();
    @keyarray = ();
    for($i = 1; $i <= $#bibitems; $i++)
	{
	$bibitems[$i] =~ s/\n$//;
	$bibitems[$i] =~ /^\s*\{([^\}\s]+)\s*\}.*/;
	$key = $1;
	push(@keyarray,$key);
	$bibhash{$key} = $bibitems[$i];
	}
    print OUT "$bibpat";
    $, = '';		# set output field separator
    foreach $key (@uniquecites)
	{
	if(exists $bibhash{$key})
	    { print OUT "\\bibitem",$bibhash{"$key"},"\n"; }
	else
	    { print "No bibitem for ", $key; }
	delete $bibhash{$key};
	}
    print OUT join("\n",@bibco) if ($#bibco != 0);
    print OUT "\\end\{references\}\n" if !$dothebib;
    print OUT "\\end\{thebibliography\}\n" if $dothebib;
    $first = 1;
    while(($key,$value) = each %bibhash)
	{
	$value =~ s/\n/\n\%/g;
	print OUT "\n\%Unused bibitems\n" if $first == 1;
	print "\n\%Unused bibitems\n" if $first == 1;
	$first = 0;
	print OUT "\%","\\bibitem",$value;
	print "\%","\\bibitem",$value;
	}
    $lastpart = $fileparts[2];
    $lastpart =~ s/\n$//;
    $lastpart =~ s/^\n+//;
    print OUT $lastpart;
    close OUT;
    `mv sortbib.tmp $file`;
    }

